An Inverse Problem Approach for Content Popularity Estimation

The Internet increasingly focuses on content, as exemplified by the now popular Information Centric Networking paradigm. This means, in particular, that estimating content popularities becomes essential to manage and distribute content pieces efficiently. In this paper, we show how to properly estimate content popularities from a traffic trace. Specifically, we consider the problem of the popularity inference in order to tune content-level performance models, e.g. caching models. In this context, special care must be brought on the fact that an observer measures only the flow of requests, which differs from the model parameters, though both quantities are related by the model assumptions. Current studies, however, ignore this difference and use the observed data as model parameters. In this paper, we highlight the inverse problem that consists in determining parameters so that the flow of requests is properly predicted by the model. We then show how such an inverse problem can be solved using Maximum Likelihood Estimation. Based on two large traces from the Orange network and two synthetic datasets, we eventually quantify the importance of this inversion step for the performance evaluation accuracy.

==> figs/hr_otu_vs_naive.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5040.00,2448.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(577,563){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(577,898){\makebox(0,0)[r]{\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(577,1233){\makebox(0,0)[r]{\strut{} 0.4}}%
      \csname LTb\endcsname%
      \put(577,1567){\makebox(0,0)[r]{\strut{} 0.6}}%
      \csname LTb\endcsname%
      \put(577,1902){\makebox(0,0)[r]{\strut{} 0.8}}%
      \csname LTb\endcsname%
      \put(577,2237){\makebox(0,0)[r]{\strut{} 1}}%
      \csname LTb\endcsname%
      \put(682,387){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1490,387){\makebox(0,0){\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(2299,387){\makebox(0,0){\strut{} 0.4}}%
      \csname LTb\endcsname%
      \put(3107,387){\makebox(0,0){\strut{} 0.6}}%
      \csname LTb\endcsname%
      \put(3916,387){\makebox(0,0){\strut{} 0.8}}%
      \csname LTb\endcsname%
      \put(4724,387){\makebox(0,0){\strut{} 1}}%
      \put(174,1400){\rotatebox{-270}{\makebox(0,0){\strut{}\scriptsize Hit Ratio}}}%
      \put(2703,123){\makebox(0,0){\strut{}\scriptsize Relative Cache Size}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(4136,890){\makebox(0,0)[r]{\strut{}\scriptsize GT}}%
      \csname LTb\endcsname%
      \put(4136,714){\makebox(0,0)[r]{\strut{}\scriptsize Naive}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figs/hr_otu_vs_naive}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figs/hr_otu_vs_nonpar.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5040.00,2448.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,704){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(726,1000){\makebox(0,0)[r]{\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(726,1296){\makebox(0,0)[r]{\strut{} 0.4}}%
      \csname LTb\endcsname%
      \put(726,1591){\makebox(0,0)[r]{\strut{} 0.6}}%
      \csname LTb\endcsname%
      \put(726,1887){\makebox(0,0)[r]{\strut{} 0.8}}%
      \csname LTb\endcsname%
      \put(726,2183){\makebox(0,0)[r]{\strut{} 1}}%
      \csname LTb\endcsname%
      \put(858,484){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1615,484){\makebox(0,0){\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(2372,484){\makebox(0,0){\strut{} 0.4}}%
      \csname LTb\endcsname%
      \put(3129,484){\makebox(0,0){\strut{} 0.6}}%
      \csname LTb\endcsname%
      \put(3886,484){\makebox(0,0){\strut{} 0.8}}%
      \csname LTb\endcsname%
      \put(4643,484){\makebox(0,0){\strut{} 1}}%
      \put(220,1443){\rotatebox{-270}{\makebox(0,0){\strut{}\scriptsize Hit Ratio}}}%
      \put(2750,154){\makebox(0,0){\strut{}\scriptsize Relative Cache Size}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3920,1317){\makebox(0,0)[r]{\strut{}\scriptsize GT}}%
      \csname LTb\endcsname%
      \put(3920,1097){\makebox(0,0)[r]{\strut{}\scriptsize Naive}}%
      \csname LTb\endcsname%
      \put(3920,877){\makebox(0,0)[r]{\strut{}\scriptsize NP}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figs/hr_otu_vs_nonpar}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figs/hr_pareto_vs_nonpar.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5040.00,2448.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,704){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(726,1074){\makebox(0,0)[r]{\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(726,1444){\makebox(0,0)[r]{\strut{} 0.4}}%
      \csname LTb\endcsname%
      \put(726,1813){\makebox(0,0)[r]{\strut{} 0.6}}%
      \csname LTb\endcsname%
      \put(726,2183){\makebox(0,0)[r]{\strut{} 0.8}}%
      \csname LTb\endcsname%
      \put(858,484){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1615,484){\makebox(0,0){\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(2372,484){\makebox(0,0){\strut{} 0.4}}%
      \csname LTb\endcsname%
      \put(3129,484){\makebox(0,0){\strut{} 0.6}}%
      \csname LTb\endcsname%
      \put(3886,484){\makebox(0,0){\strut{} 0.8}}%
      \csname LTb\endcsname%
      \put(4643,484){\makebox(0,0){\strut{} 1}}%
      \put(220,1443){\rotatebox{-270}{\makebox(0,0){\strut{}\scriptsize Hit Ratio}}}%
      \put(2750,154){\makebox(0,0){\strut{}\scriptsize Relative Cache Size}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3920,2010){\makebox(0,0)[r]{\strut{}\scriptsize GT}}%
      \csname LTb\endcsname%
      \put(3920,1790){\makebox(0,0)[r]{\strut{}\scriptsize Naive}}%
      \csname LTb\endcsname%
      \put(3920,1570){\makebox(0,0)[r]{\strut{}\scriptsize NP}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figs/hr_pareto_vs_nonpar}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figs/pareto_just_peaks.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5040.00,2736.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(990,1055){\makebox(0,0)[r]{\strut{}\scriptsize $10^{-8}$}}%
      \csname LTb\endcsname%
      \put(990,1419){\makebox(0,0)[r]{\strut{}\scriptsize $10^{-6}$}}%
      \csname LTb\endcsname%
      \put(990,1784){\makebox(0,0)[r]{\strut{}\scriptsize $10^{-4}$}}%
      \csname LTb\endcsname%
      \put(990,2148){\makebox(0,0)[r]{\strut{}\scriptsize $10^{-2}$}}%
      \csname LTb\endcsname%
      \put(1122,484){\makebox(0,0){\strut{}\scriptsize $10^{-1}$}}%
      \csname LTb\endcsname%
      \put(1920,484){\makebox(0,0){\strut{}\scriptsize $10^{0}$}}%
      \csname LTb\endcsname%
      \put(2717,484){\makebox(0,0){\strut{}\scriptsize $10^{1}$}}%
      \csname LTb\endcsname%
      \put(3515,484){\makebox(0,0){\strut{}\scriptsize $10^{2}$}}%
      \csname LTb\endcsname%
      \put(4312,484){\makebox(0,0){\strut{}\scriptsize $10^{3}$}}%
      \put(484,1587){\rotatebox{-270}{\makebox(0,0){\strut{}\scriptsize Probability}}}%
      \put(2882,154){\makebox(0,0){\strut{}\scriptsize Popularity}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1980,1537){\makebox(0,0)[r]{\strut{}\scriptsize GT (Peaks)}}%
      \csname LTb\endcsname%
      \put(1980,1317){\makebox(0,0)[r]{\strut{}\scriptsize Peaks}}%
      \csname LTb\endcsname%
      \put(1980,1097){\makebox(0,0)[r]{\strut{}\scriptsize GT (NP)}}%
      \csname LTb\endcsname%
      \put(1980,877){\makebox(0,0)[r]{\strut{}\scriptsize NP}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figs/pareto_just_peaks}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figs/pareto_mixed.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3744.00,2448.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,563){\makebox(0,0)[r]{\strut{}$10^{-10}$}}%
      \csname LTb\endcsname%
      \put(682,901){\makebox(0,0)[r]{\strut{}$10^{-8}$}}%
      \csname LTb\endcsname%
      \put(682,1239){\makebox(0,0)[r]{\strut{}$10^{-6}$}}%
      \csname LTb\endcsname%
      \put(682,1576){\makebox(0,0)[r]{\strut{}$10^{-4}$}}%
      \csname LTb\endcsname%
      \put(682,1914){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \csname LTb\endcsname%
      \put(787,387){\makebox(0,0){\strut{}$10^{0}$}}%
      \csname LTb\endcsname%
      \put(1587,387){\makebox(0,0){\strut{}$10^{1}$}}%
      \csname LTb\endcsname%
      \put(2387,387){\makebox(0,0){\strut{}$10^{2}$}}%
      \csname LTb\endcsname%
      \put(3187,387){\makebox(0,0){\strut{}$10^{3}$}}%
      \put(174,1400){\rotatebox{-270}{\makebox(0,0){\strut{}Probability}}}%
      \put(2107,123){\makebox(0,0){\strut{}Number of Requests}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1312,1242){\makebox(0,0)[r]{\strut{}\ssz GT}}%
      \csname LTb\endcsname%
      \put(1312,1066){\makebox(0,0)[r]{\strut{}\ssz NP}}%
      \csname LTb\endcsname%
      \put(1312,890){\makebox(0,0)[r]{\strut{}\ssz Naive}}%
      \csname LTb\endcsname%
      \put(1312,714){\makebox(0,0)[r]{\strut{}\ssz Zipf}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figs/pareto_mixed}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figs/pareto_mixed_head.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3744.00,2448.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(577,563){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(577,898){\makebox(0,0)[r]{\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(577,1233){\makebox(0,0)[r]{\strut{} 0.4}}%
      \csname LTb\endcsname%
      \put(577,1567){\makebox(0,0)[r]{\strut{} 0.6}}%
      \csname LTb\endcsname%
      \put(577,1902){\makebox(0,0)[r]{\strut{} 0.8}}%
      \csname LTb\endcsname%
      \put(577,2237){\makebox(0,0)[r]{\strut{} 1}}%
      \csname LTb\endcsname%
      \put(682,387){\makebox(0,0){\strut{} 1}}%
      \csname LTb\endcsname%
      \put(987,387){\makebox(0,0){\strut{} 2}}%
      \csname LTb\endcsname%
      \put(1292,387){\makebox(0,0){\strut{} 3}}%
      \csname LTb\endcsname%
      \put(1597,387){\makebox(0,0){\strut{} 4}}%
      \csname LTb\endcsname%
      \put(1902,387){\makebox(0,0){\strut{} 5}}%
      \csname LTb\endcsname%
      \put(2208,387){\makebox(0,0){\strut{} 6}}%
      \csname LTb\endcsname%
      \put(2513,387){\makebox(0,0){\strut{} 7}}%
      \csname LTb\endcsname%
      \put(2818,387){\makebox(0,0){\strut{} 8}}%
      \csname LTb\endcsname%
      \put(3123,387){\makebox(0,0){\strut{} 9}}%
      \csname LTb\endcsname%
      \put(3428,387){\makebox(0,0){\strut{} 10}}%
      \put(174,1400){\rotatebox{-270}{\makebox(0,0){\strut{}Probability}}}%
      \put(2055,123){\makebox(0,0){\strut{}Number of Requests}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2840,2086){\makebox(0,0)[r]{\strut{}\ssz GT}}%
      \csname LTb\endcsname%
      \put(2840,1910){\makebox(0,0)[r]{\strut{}\ssz NP}}%
      \csname LTb\endcsname%
      \put(2840,1734){\makebox(0,0)[r]{\strut{}\ssz Naive}}%
      \csname LTb\endcsname%
      \put(2840,1558){\makebox(0,0)[r]{\strut{}\ssz Zipf}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figs/pareto_mixed_head}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figs/vod_mixing.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(5040.00,2448.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1122,719){\makebox(0,0)[r]{\strut{}\scriptsize $10^{-10}$}}%
      \csname LTb\endcsname%
      \put(1122,1034){\makebox(0,0)[r]{\strut{}\scriptsize $10^{-8}$}}%
      \csname LTb\endcsname%
      \put(1122,1348){\makebox(0,0)[r]{\strut{}\scriptsize $10^{-6}$}}%
      \csname LTb\endcsname%
      \put(1122,1663){\makebox(0,0)[r]{\strut{}\scriptsize $10^{-4}$}}%
      \csname LTb\endcsname%
      \put(1122,1978){\makebox(0,0)[r]{\strut{}\scriptsize $10^{-2}$}}%
      \csname LTb\endcsname%
      \put(1254,484){\makebox(0,0){\strut{}\scriptsize $10^{-1}$}}%
      \csname LTb\endcsname%
      \put(1975,484){\makebox(0,0){\strut{}\scriptsize $10^{0}$}}%
      \csname LTb\endcsname%
      \put(2696,484){\makebox(0,0){\strut{}\scriptsize $10^{1}$}}%
      \csname LTb\endcsname%
      \put(3418,484){\makebox(0,0){\strut{}\scriptsize $10^{2}$}}%
      \csname LTb\endcsname%
      \put(4139,484){\makebox(0,0){\strut{}\scriptsize $10^{3}$}}%
      \put(484,1443){\rotatebox{-270}{\makebox(0,0){\strut{}\scriptsize Probability}}}%
      \put(2948,154){\makebox(0,0){\strut{}\scriptsize Popularity}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1980,1097){\makebox(0,0)[r]{\strut{}\scriptsize NP}}%
      \csname LTb\endcsname%
      \put(1980,877){\makebox(0,0)[r]{\strut{}\scriptsize Naive}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figs/vod_mixing}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> notation.tex <==
\let\proof\relax 
\let\endproof\relax
\RequirePackage{xparse}
\RequirePackage{dsfont}
\RequirePackage{amsthm}

\newcommand{\ssz}{\scriptsize}


 \DeclareMathOperator*{\argmin}{arg\,min}
 \DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\dd}{\mathrm{d}}

\newcommand{\rec}[1]{\frac{1}{#1}}

\newcommand{\mini}{\wedge}

\newcommand{\maxi}{\vee}           % Maximum operator

\newcommand{\N}{{\mathds{N}}}      % Natural numbers

\newcommand{\Z}{{\mathds{Z}}}      % Integer numbers

\newcommand{\RR}{{\mathds{R}}}     % Real numbers

\newcommand{\I}{{\mathds{1}}}      % Indicator Function

\newcommand{\II}[1]{{\mathds{1}\!\left\{#1\right\}}}

\newcommand{\Seq}[1]{ #1_1,\allowbreak #1_2,\allowbreak \ldots }

\newcommand{\FSeq}[2]{{#1_1, #1_2, \dotsc, #1_{#2}}}

\newcommand{\defEqual}{\overset{\text{def}}{=}}
\newcommand{\lawEqual}{\overset{\text{law}}{=}}
\newcommand{\distEqual}{\overset{\text{d}}{=}}
\newcommand{\iid}{i.i.d.\ }
\newcommand{\ie}{\emph{i.e.\ }}
\newcommand{\cdf}{c.d.f.\ }

\makeatletter
\DeclareDocumentCommand\E{m o o o o}{
	\mathds{E}%
	\def\@tempa{#4} \ifx\@tempa\@empty\relax{}\else \IfNoValueF{#4}{_{#4}}\fi
	\def\@tempa{#5} \ifx\@tempa\@empty\relax{}\else \IfNoValueF{#5}{^{#5}}\fi
	\!\left[
		#1
		\def\@tempa{#2} \ifx\@tempa\@empty\relax{}\else \IfNoValueF{#2}{\, | \, #2} \fi
		\def\@tempa{#3} \ifx\@tempa\@empty\relax{}\else \IfNoValueF{#3}{\, ; \, #3} \fi
	\right]
}

\DeclareDocumentCommand\PP{m o o o o o}{
	\mathds{P}%
	\def\@tempa{#2} \ifx\@tempa\@empty\relax{}\else \IfNoValueF{#2}{_{#2}}\fi
	\def\@tempa{#3} \ifx\@tempa\@empty\relax{}\else \IfNoValueF{#3}{^{#3}}\fi
	\!\left[
		#1
		\def\@tempa{#4} \ifx\@tempa\@empty\relax{}\else \IfNoValueF{#4}{\, | \, #4} \fi
		\def\@tempa{#5} \ifx\@tempa\@empty\relax{}\else \IfNoValueF{#5}{\, ; \, #5} \fi
	\right]
}
\makeatother

\newcommand{\OrdStat}[3]{ #1_{#2:#3}}
\newcommand{\V}[1]{\mathbb{V}\left[#1\right]}
\newcommand{\Pset}[1]{{\mathcal{P}(#1)}}
\newcommand{\dens}{g}       % Generic density
\newcommand{\dist}{G}       % Generic distribution
\newcommand{\rdist}{\overline{\dist}} % Generic reciprocal distribution (1 - dist)
\newcommand{\RV}{Z}         % Generic random variable

\newcommand{\ParetoD}[2]{{\text{Pareto} \left( #1, #2 \right) }}
\newcommand{\ExpD}[1]{{\text{Exponential} \left( #1 \right) }}
\newcommand{\UnifD}[2]{{\text{Uniform} \left[ #1, #2 \right] }}
\newcommand{\BetaD}[2]{{\text{Beta} \left( #1, #2 \right) }}
\newcommand{\BernD}[1]{{\text{Bernoulli} \left( #1 \right)}}
\newcommand{\WeiD}[2]{{\text{Weibull} \left( #1, #2 \right)}}
\newcommand{\Poiss}[1]{{\mathcal{P}( #1 )}} % verifier
                                % avec Felipe


\newcommand{\Csize}{C}      % Cache Size

\newcommand{\NHits}{H}      % Total Number of hits

\newcommand{\NMiss}{M}      % Total Number of hits

\newcommand{\AveNMiss}{m}
\newcommand{\AveNHits}{h}

\newcommand{\ExitTime}[1]{T_{#1}}
\newcommand{\CharTime}[1]{t_{#1}}
\newcommand{\Pin}[1]{p_{in}(#1)}

\newcommand{\EffCatSize}{\CatSize_0}

\newcommand{\Reqs}{R}       % Total Number of requests

\newcommand{\Req}{\Theta}   % Variable to specify particular requests

\newcommand{\NReqs}{N}      % Number of requests for a particular document
                            % Random Variable
\newcommand{\NReqsR}{n}     % Number of requests for a particular document
                            % Realization of the previous Random Variable

\newcommand{\SmoothPar}{\rho}
\newcommand{\Par}{\theta}
\newcommand{\Supp}{x}
\newcommand{\iPar}{i}
\newcommand{\NPar}{I}
\newcommand{\iCount}{j}           % Index for Counts
\newcommand{\MaxCount}{J}         % Maximum count
\newcommand{\iDoc}{k}
\newcommand{\CatSize}{K}    % Size of the catalog
\newcommand{\ObsDoc}{\CatSize_0} % Observed documents in the trace
\newcommand{\Fam}{\mathcal{F}}
\newcommand{\Pop}{\lambda}        % Popularity
\newcommand{\EmpMeas}{\mu}        % Empirical Measure
\newcommand{\Est}[1]{\hat{#1}} % Estimator Operator
\newcommand{\HitProba}[1]{\text{HP}\!\left(#1\right)}
\newcommand{\HitRatio}{\text{HR}}
\newcommand{\MissProba}[1]{p_{#1}}
\newcommand{\np}{\mathrm{np}}
\newcommand{\nv}{\mathrm{nv}}
\newcommand{\ml}{\mathrm{ml}}
\renewcommand{\th}{^{\mathrm{th}}}
\newcommand{\WinSize}{W}

\newcommand{\lik}[2]{\ell \left( #1; \, #2 \right)}


\newcommand{\data}[1]{\texttt{\##1}}

\newtheoremstyle{pstat} % name
    {\topsep}                    % Space above
    {\topsep}                    % Space below
    {\itshape}                   % Body font
    {}                           % Indent amount
    {\scshape}                   % Theorem head font
    {:}                          % Punctuation after theorem head
    {.5em}                       % Space after theorem head
    {}  % Theorem head spec (can be left empty, meaning 'normal')
\theoremstyle{pstat}
\newtheorem*{ps}{Problem Statement}





